Synwalk -- Community Detection via Random Walk Modelling

Complex systems, abstractly represented as networks, are ubiquitous in everyday life. Analyzing and understanding these systems requires, among others, tools for community detection. As no single best community detection algorithm can exist, robustness across a wide variety of problem settings is desirable. In this work, we present Synwalk, a random walk-based community detection method. Synwalk builds upon a solid theoretical basis and detects communities by synthesizing the random walk induced by the given network from a class of candidate random walks. We thoroughly validate the effectiveness of our approach on synthetic and empirical networks, respectively, and compare Synwalk's performance with the performance of Infomap and Walktrap. Our results indicate that Synwalk performs robustly on networks with varying mixing parameters and degree distributions. We outperform Infomap on networks with high mixing parameter, and Infomap and Walktrap on networks with many small communities and low average degree. Our work has a potential to inspire further development of community detection via synthesis of random walks and we provide concrete ideas for future research.

==> sections/appx_markov_aggregation.tex <==
\section{Relation to Markov Aggregation}\label{appx:markov_aggregation}

Here, we briefly locate our cost function within the scientific literature around Markov aggregation, i.e., around the problem of replacing a random walk $\{X_t\}$ on a large state space by one on a significantly smaller state space. Several authors have proposed using the Kullback-Leibler divergence rate as a cost function for Markov aggregation~\citep{Deng2011,Geiger2015,Vidyasagar2010}. Specifically,~\citet{Deng2011} aimed at finding an aggregation function $m{:}\ \dom{X}\to\idxset{Y}$ that maximizes $\mutinf{Y_t;Y_{t-1}}$ (in the notation of this work). As we show in Appendix~\ref{appx:proofs}, this cost function is also obtained by further relaxing our Synwalk objective~\eqref{eq:si_objective}.
